Unveiling Attractor Cycles in Large Language Models: A Dynamical Systems View of Successive Paraphrasing

Dynamical systems theory provides a framework for analyzing iterative processes and evolution over time. Within such systems, repetitive transformations can lead to stable configurations, known as attractors, including fixed points and limit cycles. Applying this perspective to large language models (LLMs), which iteratively map input text to output text, provides a principled approach to characterizing long-term behaviors. Successive paraphrasing serves as a compelling testbed for exploring such dynamics, as paraphrases re-express the same underlying meaning with linguistic variation. Although LLMs are expected to explore a diverse set of paraphrases in the text space, our study reveals that successive paraphrasing converges to stable periodic states, such as 2-period attractor cycles, limiting linguistic diversity. This phenomenon is attributed to the self-reinforcing nature of LLMs, as they iteratively favour and amplify certain textual forms over others. This pattern persists with increasing generation randomness or alternating prompts and LLMs. These findings underscore inherent constraints in LLM generative capability, while offering a novel dynamical systems perspective for studying their expressive potential.

==> article/AI_homogenization.tex <==

\section{AI homogenization Posed By Successive Paraphrasing with Diverse LLMs}
\label{SPwithDiverseModel}
In this section, we extend our experiments by incorporating a variety of large language models (LLMs). At each step, for every paraphrase, we randomly select an LLM to perform the paraphrasing, thereby generating the dataset for the next step.
In our view, current general LLMs are likely to follow a similar distribution due to the substantial overlap in their pre-training and instruction-tuning datasets, as well as their similar model structures.
Therefore, we anticipate that the periodicity we previously mentioned will also manifest in this task setting.

The results presented in Appendix \ref{} are consistent with our conjecture.
Although it is less obvious than the periodicity observed with single LLMs due to the noise introduced by using diverse LLMs, this phenomenon is still present.
This indicates that the text paraphrased by each LLM still maintains a low perplexity when evaluated against other LLMs.
The results reflect that current general LLMs indeed follow a similar distribution, which we refer to as AI homogenization.
The reason for model homogenization lies in the flaws inherent in current statistical AI theory.
We can summarize current statistical AI as the use of models to approximate the distribution of a given dataset.
The prevalent LLMs (such as Chatgpt, GLM4, and Llama3 etc.) have nearly exhausted all available corpus on the internet.
This implies that the training corpora of these powerful LLMs have significant overlap.
Additionally, most current general LLMs are based on transformers and share similar underlying structures, with the exception of recent models like RWKV and Mamba, which have not yet been widely adopted.
Moreover, these LLMs are trained in similar ways, using the same loss functions, training frameworks, and other methodologies.
All these factors contribute to model homogenization, which is a significant issue today. 
%This not only challenges the rights of the models but also accelerates corpus homogenization.
%In section \ref{}, we will comprehensively discuss the potential impact of AI homogenization.

AI homogenization raises serious philosophical and copyright issues concerning AI authorship.
Philosophically speaking, if two teams independently train two models that produce similar distributions and both models generate the same article, which model should be considered the author of that article?
Additionally, due to AI homogenization, texts generated by LLMs tend to be homogeneous, making it difficult to accurately determine which model generated them.
Besides the challenges and issues mentioned above, the homogeneous responses produced by current LLMs further accelerate the homogenization of the digital environment.







==> article/ConnectionBetween2C.tex <==
\subsection{Deeper Understanding Periodicity}
\label{sec:Convergence2Periodicity}

%\textbf{Periodicity serves as an outward expression of convergence.}
The inherent characteristics of LLMs enable them to generate sequences with low perplexity, indicating a high probability of occurrence. 
During successive paraphrasing, both perplexity and reverse perplexity consistently decrease, resulting in diminished generation diversity and an increased likelihood of \(T_{i-1}\) appearing in the output space of \(T_i\). 
When the reverse perplexity approaches the perplexity, we can treat \(T_{i-1}\) and \(T_{i+1}\) as essentially equivalent. Additionally, low generation diversity suggests that the texts in \(T_{i+1}\) are highly similar to one another.
Therefore, the text in \(T_{i-1}\) may be virtually indistinguishable from the text in \(T_{i+1}\).

%In extreme cases, when \(T_{i-1}\) functions as a candidate paraphrase for \(T_i\) and the generation diversity of \(T_i\) is sufficiently low, the difference between \(T_{i-1}\) and \(T_{i+1}\) becomes minimal. 
%This is due to the reduction in reverse perplexity; as the reverse perplexity of \(T_{i-1}\) conditioned on \(T_i\) approaches that of \(T_{i+1}\) conditioned on \(T_i\), \(T_{i-1}\) qualifies as a candidate paraphrase for \(T_i\). 
%However, the intrinsic nature of paraphrasing requires LLMs to produce variations of the original text, resulting in \(T_{i+1}\) differing from \(T_i\). Combining these characteristics, LLMs perform a 2-periodicity in successive paraphrasing.




The decrease in reverse perplexity can be attributed to the invertibility of paraphrasing. 
Given a text and one of its paraphrases, we can consider the text as a paraphrase of its paraphrase, reinforcing the notion of invertibility of paraphrasing.
Building on this perspective, there are likely other tasks characterized by invertibility that exhibit similar periodicity to paraphrasing. We will extend our experiments to investigate this further in Section \ref{sec:beyond paraphrasing}.


%The nature of LLMs leads them to generate sequences with low perplexity, indicating a high likelihood at the same time.
%During successive paraphrasing, both perplexity and reverse perplexity consistently decrease, leading to a reduction in generation diversity and an increase in the likelihood of $T_{i-1}$ appearing in the output space of $T_i$.
%In an extreme situation, where the $T_{i-1}$ is a candidate paraphrase of \(T_i\) and the generation diversity of \(T_i\) is also low enough, there will be little difference between $T_{i-1}$ and $T_{i+1}$.
%Due to the decrease in reverse perplexity, when the reverse perplexity of \(T_{i-1}\) conditioned on \(T_i\) is near the perplexity of \(T_{i+1}\) conditioned on \(T_i\), T_{i-1} is in the candidate paraphrases of \(T_i\).



\iffalse

\subsection{The Mathematical Perspective}

We aim to explain that under certain conditions, the successive paraphrasing process using a LLM converges to an approximate period-2 behavior. Specifically, we incorporate the empirical findings that both forward and backward perplexities decrease as the iterative steps increase.
We represent the convergence of forward and backward perplexity as,
\[
\lim_{n\to\infty}\mathcal{L}(T_{n+1}|T_{n})=\mathcal{L}_f \geq 0    
\]
\[
\lim_{n\to\infty}\mathcal{L}(T_{n}|T_{n+1})=\mathcal{L}_b \geq 0    
\]
as both forward and backward perplexity decreases, \(P\) and \(P^{-1}\) becomes increasingly deterministic, 

Meanwhile, there exists \(\delta>0\) such that for all \(n\),
\[
d(T_{n+1},T_n) \geq \delta
\]
This ensures sufficient diversity between consecutive texts.


Under the above definitions and assumptions, the sequence \(\{T_n\}\) exhibits approximate period-2 behavior.
Specifically, there exists \(N \in Z^+\), such that for all \( n \geq N \),
\[
d(T_{n+2},d_{n}) \leq \epsilon,
\]
where \(\epsilon > 0\) is a small positive value indicating low diversity between \(T_n\) and \(T_{n+2}\). 
We will provide a brief explanation below.


\textbf{Step 1: Behavior of \(P\) and \(P^{-1}\) After Perplexity Convergence.}
Given \(P^{-1}\) represents the LLM’s mapping from a paraphrase back to the original text.
As both forward and backward perplexities decrease, the functions 
\(P\) and \(P^{-1} \) become increasingly deterministic and invertible. 
For sufficiently large \(n\), we have:
\[
P(T_n) = T_{n+1}, P^{-1}(T_{n+1}) = T_n.
\]

\textbf{Step 2: Establishing that \(P\) is an Involution.}
We will show that \(P\) is an involution on the set of texts after convergence.
Since \(P^{-1}\) is the inverse of P, and both are deterministic:
\[P^{-1}=P\]
Therefore, \(P(P(T)) = T\), for all T after convergence, which means that \(P\) is an involutive function.



\textbf{Step 3: Implications of \(P\) Being an Involution.}
Because \(P\) is an involution, its mapping consists solely of fixed points and
transpositions (cycles of length 2). 
However, the minimal dissimilarity constraint rules out fixed points (cycles of length 1), since:
\[P(T) = T \rightarrow d(T, T) = 0 < \delta\]

\textbf{Step 4: The Sequence Must Cycle Between Exactly Two Texts.}
Given that \(P\) is an involution without fixed points, the only possible cycles
are of length 2. Let \(T_A\) and \(T_B\) be the texts such that:
\[
P(T_A)=T_B, P(T_B)=T_A
\]
Thus, the sequence alternates between TA and TB:
\begin{equation*}
T_n =
\begin{cases}
    T_A, & \text{if } n \text{ is even}, \\
    T_B, & \text{if } n \text{ is odd}.
\end{cases}
\end{equation*}


\textbf{Step 5: Verifying the Minimal Dissimilarity Constraint.}
The minimal dissimilarity constraint is satisfied since:
\[d(P(Tn), Tn) = d(Tn+1, Tn) \geq \delta\]
This holds for all \(n\), as \(T_n\) and \(T_{n+1}\) are distinct due to the absence of fixed points.

\textbf{Step 6: Bounding the Distance Between \(T_{n+2}\) and \(T_n\).}
In the deterministic case, we have:
\[
T_{n+2} = P(T_{n+1}) = P(P(T_n)) = T_n.
\]
As a result:
\[
d(T_{n+2}, T_n) = d(T_n, T_n) = 0.
\]
However, in practice, residual stochasticity introduces small deviations, so we consider:
\[
d(T_{n+2}, T_n) \leq \epsilon,
\]
where \(\epsilon\) is a small positive value. This adjustment links the theoretical result to empirical observations, such as the low diversity (e.g., low normalized edit distance scores) between \(T_n\) and \(T_{n+2}\).

\textbf{Step 7: Impossibility of Longer Periods.}
Assume, for the sake of contradiction, that there exists a period \(k > 2\) with distinct texts \(T_0, T_1, \dots, T_{k-1}\) such that: \(T_{n+k} = T_n\), and \(P(T_i) = T_{i+1}\) for \(i = 0, 1, \dots, k-1 \mod k\).

Since \(P\) is deterministic and invertible (an involution), we must have:
\[
P(P(T_i)) = T_i \quad \text{for all } i.
\]
This implies:
\[
T_i = P(P(T_i)) = P(T_{i+1}) = T_{i+2}.
\]
Therefore:
\[
T_{i+2} = T_i.
\]
This means the sequence repeats every 2 steps, contradicting the assumption that the period is \(k > 2\). Thus, longer periods are impossible under the given conditions.


As we illustrate above, the only possible behavior is an approximate period-2 cycle between \(T_A\) and \(T_B\). The minimal dissimilarity constraint eliminates
fixed points, and the involutive nature of \(P\) precludes longer cycles. 
\fi


==> article/DigitalEnv.tex <==
%\section{Discussion}
%In this section, we will explore the significance and potential applications of our findings, and discuss their impact on the Internet.
%Firstly, our findings reflect the self-enhancement nature of large language models (LLMs). Secondly, these findings can be applied to defend against current successive paraphrasing attacks, leading to a more robust AI text detection system. Furthermore, we illustrate how to break out of the periodic cycle. Finally, we discuss the potential risks and impacts of the widespread utilization of LLMs for paraphrasing.
%These points will be illustrated in detail in the following subsections.
\section{Digital Environment Homogenization}
Digital environment homogenization has raised a great concern in the research community, with the widespread use of LLMs.
In this paper, We have already demonstrated how successive paraphrasing contributes to this homogenization and the inherent principal behind it.
What concerns us most is that homogenization will become even more severe as LLMs grow more powerful.
We further conducted the same experiments across a series of LLMs with well-recognized performance rankings. 
The results in Appendix \ref{} indicate that as LLMs continue to develop, they are likely to exacerbate the issue of homogenization.
We believe that current LLMs are enhancing their ability to answer factual questions with precise responses, which leads to more specific answers. 
However, this increased specificity contributes to homogenization. 
As LLMs continue to advance, the issue of homogenization will become more pronounced, resulting in a more uniform digital world, which seems like the curse of statistic AI.


We face a future where the internet is saturated with AI-paraphrased content, and whether its impacts are entirely negative needs to be discussed.


From a negative perspective, The digital environment can be likened to natural ecosystems. 
Just as a loss of biodiversity makes a natural ecosystem more vulnerable and less robust, homogenization in the digital environment can have similar weakening effects. 
The diminishing of linguistic diversity in the digital world will lead to a dilemma in preserving the complexity, resilience, and richness of our culture,  potentially reshaping the thinking of future generations. 
At an AI level, this could also influence the training of next-generation LLMs. 
The study by \citealt{} highlights the potential risk that incorporating model-generated content into the training process of future models might lead to model collapse.


From a positive perspective, however, paraphrasing tools based on LLMs have been widely used in education, news, and academic, and a series of studies have shown that they can help children learn language more effectively.
Besides, the increased presence of texts generated by LLMs aligned with human values on the internet can also help shape a positive personality in future generations, leading to a harmonious and peaceful world.
For LLMs, We can also leverage homogenization to accelerate model training. 
The web corpus, which consists of paraphrased texts rather than directly generated ones, can update factual knowledge while improving grammatical fluency. 
Utilizing these model-preferred corpora—designed to avoid repetitive memorization—may result in a more efficient training process, faster convergence due to the consistent distribution, and a reduced risk of model collapse.

%\subsection{AI Homogenization}
%\label{AI homognization}
%In Section \ref{SPwithDiverseModel}, we have pointed out the problem we refer to as AI homogenization within LLMs.
%We argue that it is caused by similar training processes, significant overlap in datasets, and similar model structures.
%AI homogenization raises serious philosophical and copyright issues concerning model rights and presents significant challenges in AI text attribution. 
%Philosophically speaking, if two teams independently train two models and these models exhibit similar distributions, can it still be said that each model possesses a unique right?
%Except the model rights, it also brings challenge in text source attribution, which means determining which AI model or system generated a specific piece of text.




==> article/Simulation.tex <==
\section{Real World Paraphrase Simulation}
Initially, we created a simulation experiment to mimic the real-world application of paraphrasing.
In the real world, new human-written and LLM-paraphrased texts are constantly being added to the internet. The text that LLMs paraphrase can often be content that has already been paraphrased by LLMs, sometimes multiple times, for various reasons.
To simulate this scenario, we started by creating a corpus of 1,000 texts. 
At each step, we paraphrased 100 of those texts and added 100 new texts to the corpus.
We sampled 1,000 texts from each stage of the corpus and calculated the perplexity distribution. 
The results \ref{} indicate that the distribution of the corpus became progressively more concentrated over time.









                                                                                                                                                                  

==> article/Solutions.tex <==

\subsection{Mitigating Generation Momentum}


% \section{Discussion}

% Understanding LLM Generation Momentum from the Lens of Successive Paraphrasing
% different models


% \textbf{Homogenization is the curse of LLMs.} 
% From the macro perspective, homogenization is lacking in the current statistic AI theory.
% In the current research community, the performance of an LLM is evaluated through a series of benchmarks.
% If one LLM outperforms another, it should achieve better results across these benchmarks, indicating that its responses are more accurate. However, focusing on improving response accuracy can reduce the richness and diversity of responses, leading to greater homogenization.
% Current LLMs aim to approximate real-world distributions based on a given corpus, consuming almost all available data on the internet. Given a specific corpus, we assume that there exists an optimal LLM within the current theoretical framework.
% From a micro perspective, the significant overlap in training datasets, similar training processes, model structures, and objectives will cause the LLMs to learn from similar distributions, leading to AI homogenization, which is the main contribution to the \textbf{DEH}.
% Furthermore, the limitations of the decoding strategy restrict the expressive capabilities of LLMs, intensifying the issue of \textbf{DEH}.

% \textbf{Relieve homogenization}


% \textbf{Relieve digital environment homogenization caused by S.P.} 
% do not fix a specific prompt, 
% adding noise to text
% adding system prompt




==> article/convergence_to_periodicity.tex <==
\section{The Connection Between Periodicity and Convergence}
Periodicity serves as an outward expression of convergence.
In this section, we will explore this idea from both an intuitive and mathematical perspective.
\label{Convergences2Periodicity}
\subsection{An intuitive perspective to understand the periodicity in SP}
The nature of LLMs leads them to generate sequences with low perplexity, indicating a high likelihood at the same time.
Recalling that an SP process can be represented as \((s_1, s_2, \dots, s_n)\), we define the set of all SP processes as \(\Omega = \{SP_1, SP_2, \dots, SP_n\}\). The paraphrased corpus at the \(i\)th step is defined as \(SP_j = \{SP_{ji} \mid SP_j \in \Omega\}\).
Let's consider an extreme case.
If the reverse condition perplexity and the condition perplexity converge at the same value \(\alpha\), we can think step corpus \(S_{i-1}\) and \(S_{i+1}\) follow the same distribution.
Specifically, this means that both \(S_{i-1}\) and \(S_{i+1}\) can be derived from \(S_i\) through paraphrasing. 
Since \(S_{i+1}\) is indeed derived from \(S_i\), we can rephrase the claim more concisely: \(S_{i-1}\) can also be derived from \(S_i\). 
If not, the subsequent corpus \(S_{i+1}\) derived from \(S_i\) must have lower conditional perplexity, as LLMs tend to generate sequences with low perplexity, which counters our assumption.
So, in this situation, during a successive paraphrase process, when \(i\) becomes sufficiently large, \(s_{i-1}\) and \(s_{i+1}\) are within the sample space of \(s_i\).
When \(\alpha\) is sufficiently low, the similarity between \(s_{i-1}\) and \(s_{i+1}\) is high, leading to a periodic pattern in the entire paraphrase corpus sequences.

\subsection{A mathematical perspective to understand the periodicity in SP}

In this section, we explain how convergence leads to periodicity during successive paraphrasing. We define the similarity function as \(\Omega\), the conditional perplexity function as \(\sigma\), and the distribution of successive paraphrasing as \(p\). The convergence of conditional perplexity during successive paraphrasing (SP) can be represented as:
\[
E_{t_{i+1}, t_{i} \sim p}[\sigma(t_{i+1}|t_{i})] < E_{t_{i}, t_{i-1} \sim p}[\sigma(t_{i}|t_{i-1})], \quad \lim_{i \to \infty} E_{t_{i}, t_{i-1} \sim p}[\sigma(t_{i}|t_{i-1})] = \alpha
\]
\[
\sigma(t_{i+1}, t_{i}) = \exp \left( -\frac{1}{T} \sum_{j=1}^{T} \log P(t_j \mid t_i, t_{i+1}^1, t_{i+1}^2, \ldots, t_{i+1}^{j-1}) \right)
\]
Meanwhile, We believe that the characteristics we have mentioned are inherent to LLMs. The key to periodicity is the task-specific decrease in reverse conditional perplexity, which can be represented as:

\[ E_{t_{i-1},t_{i} \sim p}[\sigma(t_{i-1}|t_{i})] - E_{t_{i+1},t_{i} \sim p}[\sigma(t_{i+1}|t_{i})]<\theta \\\lim_{i\to \infty} E_{t_{i-1},t_{i} \sim p}[\sigma(t_{i-1}|t_{i})]  < \alpha+\theta \]

As the conditional perplexity decreases, the similarity increases, showing a positive correlation with the conditional perplexity. Formally, this can be represented as:
\[
E_{t^1_{i+1}, t^2_{i+1}, t_i \sim \gamma}[\Omega(t^1_{i+1}, t^2_{i+1})] = 1 - kE_{t_{i+1}, t_{i} \sim p}[\sigma(t_{i+1}|t_{i})]
\]
This means that when the perplexity is low if you derive two paraphrases from a text, these two paraphrases will exhibit a high degree of similarity with each other. 
To simplify the deduction, while the conditional perplexity is low, we approximate this as:
\[ \forall t_{i+1}^1,t_{i+1}^2 \in M_p(*|t_{i}),\quad  \Omega(t^1_{i+1},t^2_{i+1})=1-k\alpha\]

We define all possible paraphrases of \(t_i\) as \(\hat{T}_{i+1}\) in the real world. The set \(T_{i+1}\) generated by LLMs should be a subset of \(\hat{T}_{i+1}\), containing elements that exhibit low conditional perplexity. Formally, we define:
\[
T_{i+1} = \{t_{i+1} \mid |\sigma(t_{i+1}, t_i) - \alpha| \le \epsilon, t_{i+1} \in \hat{T}_{i+1}\}
\]

While the number of step is high enough, Our goal is to prove that:
\[E_{t_{i-1}, t_{i+1} \sim p}[\Omega(t_{i-1}, t_{i+1})] > \Theta\]
where \(\Theta\) is sufficiently high, which means the \(T_{i+1}\) is very similar to \(T_{i-1}\).

It can be proven that:
\[E_{t_{i-1},t_{i+1} \sim p}[\Omega(t_{i-1},t_{i+1})] > (1-k\alpha)(1-\frac{\beta-\alpha}{\theta})\]
And we put the detailed proof in the Appendix \ref{}. It shows that while the reverse conditional perplexity is approaching the conditional perplexity, and the conditional perplexity is low, it will show the periodicity, the \(T_{i+1}\) is very similar to \(T_{i-1}\), which can properly explain our phenomenon.

%In this section, we will explain how the convergence causes the periodicity during successive paraphrasing.
%We define the similarity function as \(\Omega\), the condition perplexity function as \(\sigma\), and the distribution of successive paraphrasing as \(p\). The convergence of condition perplexity during SP can be represented as:
%\[
%E_{t_{i+1},t_{i} \sim p}[\sigma(t_{i+1}|t_{i})] < E_{t_{i},t_{i-1} \sim p}[\sigma(t_{i}|t_{i-1})],  \lim_{i \to \infty} E_{t_{i},t_{i-1} \sim p}[\sigma(t_{i}|t_{i-1})] =\alpha \\ 
%\]
%\[\sigma(t_{i+1},t_{i}) = \exp \left( -\frac{1}{T} \sum_{j=1}^{T} \log P(t_j \mid t_i, t_{i+1}^1, t_{i+1}^2, \ldots, t_{i+1}^{j-1}) \right)\]
%While the conditional perplexity decreases, the similarity also increases and shows a positive correlation with the conditional perplexity. Strictly, it can be represented as:
%\[E_{t^1_{i+1},t^2_{i+1},t_i\sim \gamma}[\Omega(t^1_{i+1},t^2_{i+1})]=1-kE_{t_{i+1},t_{i} \sim p}[\sigma(t_{i+1}|t_{i})\]
%This means while the perplexity is low if you derive 2 paraphrases from a text, the 2 paraphrases show a high similarity with each other.


\section{Generalization Analysis}

\subsection{Beyond Paraphrasing}

According to our deduction, periodicity should exist in tasks where the reverse conditional perplexity decreases as the number of steps increases. Intuitively, these tasks—where we assume \(t_i\) is derived from \(t_{i+1}\) and the concatenation of \(t_{i+1}\) and \(t_i\) is fluent—should exhibit periodicity.
To further support our theory, we designed several tasks and observed their periodicity. 
The tasks we designed are shown in Table \ref{table:other_taks}.

\begin{table*}[h!]
\centering
\begin{tabular}{|p{3cm}|p{3cm}|p{3cm}|p{3cm}|}
\hline
\textbf{Polish} & \textbf{Style Transfer} & \textbf{Formalize} & \textbf{Translation} \\ \hline
Please paraphrase the following text: & Transform the following formal text into an informal, conversational style; Rewrite the following informal text in a formal style & Rewrite the following informal text in a formal style & Please translate the following English to Chinese; Please translate the following English to Chinese;
\\ \hline
\end{tabular}
\label{table:other_taks}
\caption{Tasks}
\end{table*}

The results of these tasks are displayed in Appendix \ref{}. All of these tasks show the same periodicity, which strongly supports our deductions.



\subsection{Alternating Models and Prompts}


In this section, we extend our experiments to include variations in both the LLMs and the prompt settings.
During the \textbf{S.P.} process, for the LLM variation setting, we randomly select an LLM and apply a specific prompt. Conversely, for the prompt variation setting, we randomly choose a prompt and apply it to a specific LLM.
Despite the increased complexity in these settings, periodicity shown in figure \ref{} still remains evident.


Currently, there are several paraphrasing tools based on LLMs that primarily paraphrase the user's text with a fixed prompt. 
The periodicity observed in prompt varied \textbf{S.P.}, indicates the limited expressive range of these LLMs and illustrates how the widespread use of these paraphrasing tools can contribute to digital world homogenization.

Meanwhile, The periodicity observed in model variation \textbf{S.P.} suggests a homogenization within current LLMs. We've discussed that low perplexity is crucial for periodicity, and this experiment demonstrates that paraphrasing generated by one LLM still exhibits low perplexity on other LLMs. Given that LLMs generally produce low-perplexity text, this phenomenon implies that all LLMs share a similar output distribution in the \textbf{S.P.} task, implicitly pointing to the homogenization of LLMs.
This makes it extremely challenging to attribute AI-generated texts to the specific LLMs that produced them, and the homogenization of LLMs could further accelerate the homogenization of the digital environment.


% \subsection{Paragraph Paraphrase}


\subsection{Human Intervention}



==> article/data_collection.tex <==
\section{Data Collection}
We conducted our experiment in both English and Chinese settings. 
We collected 800 English texts from arXiv, Quora, Wiki, and CNN news in equal proportions to form a original English text dataset.
For Chinese, We randomly selected 800 Chinese translations from WMT2019.
Both datasets were recursively paraphrased 15 times by the current widely used LLMs respectively. 
Additionally, we tested four different prompts to further explore the universality of our findings.
Table 1 shows the details of our experiment setting.
\begin{table*}[h!]
\centering
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{arXiv} & \textbf{Quora} & \textbf{Wiki} & \textbf{CNN} & \textbf{WMT2019} \\
\midrule
Original & 200 & 200 & 200 & 200 & 800 \\
chatgpt & 3000 & 3000 & 3000 & 3000 &- \\
llama3-8B-chat & 3000 & 3000 & 3000 & 3000 &- \\
Mistral & 3000 & 3000 & 3000 & 3000 &- \\
GLM4-chat & 3000 & 3000 & 3000 & 3000 & 12000 \\
Baichuan3-Turbo & 3000 & 3000 & 3000 & 3000 & 12000 \\
\bottomrule
\end{tabular}
\caption{Model and Text Number Information.The paraphrase text number is determined by multiplying the number of stages by the number of texts in each stage. }
\label{table:model_text_number_info}
\end{table*}


==> article/intro_v3.tex <==
\section{Introduction}



==> article/introduction_v2.tex <==
\section{Introduction}



% LLM advantage
% paraphrase generation -> successive
% what pattern?
% how to escape

Paraphrases are sentences or phrases that convey the same meaning using different wording\citep{bhagat2013what}.
With the advancement of large language models (LLMs) ~\citep{llama,gpt3,gpt4}, paraphrasing has gained widespread use, leading to the emergence of numerous online paraphrasing tools powered by these models. 
These tools have become particularly popular for refining articles and posts, especially among non-native speakers.
So far, many researchers have focused on the misuse of paraphrasing, including plagiarism \citep{plagiarism} and the spread of fake news \citep{detect-gpt}.
Besides, Some research shows that paraphrased texts also suffer from issues like hallucination \citep{llm_hallu,llm_hallu2} and bias \citep{llm_bias}.
Other researchers have explored a more practical scenario known as successive paraphrasing (SP), where a text is paraphrased multiple times by different individuals for various reasons. 
\cite{can_ai} investigates how SP can evade current AI text detection methods, while \cite{ship} discusses the impact of SP on determining authorship.
Our research stands out from existing work in the field of paraphrasing. 
By analyzing the effects of successive paraphrasing, we identify risks associated with the evolution of LLMs, which we refer to as \textbf{Digital Environment Homogenization} and the underlying \textbf{AI Homogenization}.


Digital environment homogenization (DEH) has recently become a significant concern.
As AI systems generate language based on pre-existing user data and interactions, there is a risk that they could perpetuate and even amplify existing linguistic norms and biases, resulting in the homogenization of language \citep{homogenization}.
\cite{anderson2024homogenization} shows that LLMs exert a stronger homogenizing effect on creative works compared to humans. 
Additionally, \cite{deepfake} highlights the distinct distribution of LLM-generated text in contrast to human-written text. 
%As large language models (LLMs) are increasingly used, the internet is gradually becoming saturated with machine-generated texts. 
As noted by \cite{shumailov2023curse}, the corpora mixed with these LLM-generated texts can lead to model collapse during the training process.
So, digital environment homogenization could have a profound impact on the development of next-generation LLMs.
Moreover, a digitally homogenized world could reshape the thinking of future generations, potentially passing on inherent stereotypes to them \citep{kotek2023gender,shrawgi-etal-2024-uncovering}.

%\textbf{Successive paraphrasing leading to DEH, and simulation experiments}
To clearly illustrate the homogenizing effect caused by the widespread use of paraphrasing, we conduct a simplified experiment that simulates the real digital environment in which people consistently produce paraphrased content by using LLMs.
We use several widely adopted commercial LLMs to paraphrase a subset of the corpus at each step, while concurrently adding new human-generated texts.
At each step, we calculate the standard deviation of the perplexity of the corpus.
Details of the simulation experiment setup can be found in Appendix \ref{Simulation}.
The results shown in \ref{intro} indicate that as the number of steps increases, the standard deviation of perplexity decreases significantly, implicitly revealing the potential homogenization issue in the future.
To understand the underlying causes of homogenization, we designed various experiments to explore successive paraphrasing and identified two interesting characteristics: periodicity and convergence.

%\textbf{Periodicity and Convergence}
Assuming a successive paraphrasing (SP) process denoted as \( s_{1}, \dots, s_{n} \), the periodicity of SP refers to the pattern observed when \( s_{i+1} \) shows significant grammatical similarity to \( s_{i-1} \) during the paraphrasing sequence. 
This suggests that LLMs have limited expressive diversity, which significantly contributes to \textbf{DEH}.
Additionally, we conduct a deeper analysis of the generation process and identify convergence phenomena occurring during the \textbf{SP} process. 
As the step number increases, the perplexity of paraphrase \( s_{i} \) conditioned on \( s_{i-1} \) or \( s_{i+1} \) decreases inversely. 
We identify an intrinsic connection between convergence and periodicity, and we discuss how convergence gives rise to periodicity from both an intuitive and mathematical perspective.
Based on our deduction, we propose a series of tasks that exhibit periodicity, which strongly supports our reasoning.
Furthermore, we conduct the \textbf{S.P.} under the model and prompt variations settings, and it still performs the periodicity characteristic.
It also indicates the underlying homogenization in current LLMs which we refer to \textbf{AIH}.


In the end, we examine the potential effects of \textbf{DEH} and \textbf{AIH}. 
 We consider AIH an inevitable challenge in LLM theory, a view strongly supported by S.P.'s experiments.
In the current theoretical model, improving LLMs could exacerbate the issue of homogenization. 
Therefore, We propose several potential solutions to reduce these risks and discuss the path toward developing more creative LLMs.



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{article/figs_v1/intro.png}
    \caption{The similarity confusion matrix of successive paraphrasing is depicted in the following figures. Figures (a), (b), (c), and (d) illustrate the similarity confusion matrix for English successive paraphrasing, whereas figures (e) and (f) display the matrix for Chinese.} 
    \label{intro}
\end{figure}



==> article/introduction_v3.tex <==

\section{Introduction}
%In recent years, large language models (LLMs) have experienced rapid development. 
%Current LLMs demonstrate their impressive language abilities and have been widely used in people's daily lives, especially for polishing or rewriting articles, which has been extensively investigated in the research community and is referred to as paraphrasing ~\citep{bhagat2013what}.
%Using LLMs to paraphrase text is not only a great way to polish articles, especially for non-native speakers, but also an efficient method for data augmentation.
%However, some research also poses that potential misuse of paraphrasing might lead to plagiarism and the spread of fake news. 
%Besides, these texts paraphrased by LLMs might suffer from hallucinations\cite{} and factual errors\cite{}.

Paraphrases are sentences or phrases that convey the same meaning using different wording\citep{bhagat2013what}. 
Current large language models (LLMs) have demonstrated impressive ability in paraphrasing and have been widely used to polish articles and posts, especially for non-native speakers. 
In the research community, paraphrasing is also an efficient method for data augmentation\cite{}, helping solve the low resource problems\cite{}. 
However, some research also poses that potential misuse of paraphrasing might lead to plagiarism and the spread of fake news. 
Besides, these texts paraphrased by LLMs might suffer from hallucinations\cite{} and factual errors\cite{}.
Although there has been a considerable amount of work focusing on paraphrasing, most of it only considers text that has been paraphrased once.
In the real world, due to the widespread use of LLMs, any text you read on the internet might have been edited and paraphrased multiple times by various individuals for different reasons, a process we refer to as successive paraphrasing.
Based on our intuition and daily use of LLMs, we have noticed that successive paraphrasing exhibits some unique properties which raise our great interest.



We conduct our experiments using 2 language settings: English and Chinese. 
We collected 800 texts from \textbf{arXiv}, \textbf{Quora}, \textbf{Wikipedia}, and \textbf{CNN News} in equal proportions to form the original English dataset.
For the Chinese dataset, we sampled 800 texts from WMT2019\cite{}.
Each text in the datasets will be paraphrased 15 times by various LLMs (e.g., GPT-3.5-turbo, Llama3-8B-instruct, and GLM4-9b-chat). 
We calculate the BLEU score within each step paraphrase, and the result demonstrates that all LLMs exhibit periodicity during successive paraphrasing. 
The periodicity of successive paraphrases indicates that when you repeatedly paraphrase a text, each paraphrase is more similar to the one made two steps earlier. 
This implies that the nth paraphrase exhibits higher similarity with the (n-2)th, (n-4)th, (n-6)th, and so forth.



Moreover, through our comprehensive investigation, we reveal that successive paraphrasing tends to converge across various dimensions. 
To evaluate the diversity of potential paraphrased texts, we introduce a metric called sample space diversity. 
As the number of paraphrase steps increases, the resulting text becomes more certain, as indicated by the declining trend in sample space diversity (SSD). 
Meanwhile, the perplexity of paraphrases shows a decreasing trend and eventually converges to a specific value.
Besides, we show that there exists a strong positive correlation between SSD and perplexity in successive paraphrasing.
Furthermore, we argue that the periodicity observed in successive paraphrasing may be attributed to convergence phenomena. 
We believe that the low perplexity of the text being paraphrased is key to this periodicity.
In section 5, we will elaborate in detail how the convergence leads to periodicity.


While periodicity emerges during successive English paraphrasing by ChatGPT, the successive Chinese paraphrases show little periodicity. 
In our opinion, this is also the evidence supporting our hypothesis.
Since English occupies the largest proportion of the training corpus for ChatGPT, the model tends to have lower perplexity when processing English compared to Chinese.
To further support our assumption, we employed different LLMs to generate 10 samples at each iteration, selecting samples with the highest and lowest perplexity for the subsequent paraphrasing step.
The experiment's outcome shows the connection between perplexity and periodicity of successive paraphrasing.


Based on these properties, we discuss the potential use and harm of successive paraphrasing.
%%%%%


%%%%%%


Overall, in this paper, we deeply investigated the properties of successive paraphrasing. Our contributions are summarized as follows:
\begin{itemize}
    \item To our knowledge, we are the first to comprehensively study successive paraphrasing across a range of widely used large language models and identify the inherent periodicity and convergence.
    
    \item We propose a hypothesis that the periodicity observed in successive paraphrasing might be attributed to convergence phenomena and present experiments to support our view.
    \item We discuss the potential use and harm of successive paraphrasing.   
\end{itemize}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{article/figs_v1/intro.png}
    \caption{The similarity confusion matrix of successive paraphrasing is depicted in the following figures. Figures (a), (b), (c), and (d) illustrate the similarity confusion matrix for English successive paraphrasing, whereas figures (e) and (f) display the matrix for Chinese.}  
\end{figure}
%We discovered that successive paraphrases demonstrate both \textbf{periodicity} and \textbf{convergence}.
%The periodicity of successive paraphrases indicates that when you repeatedly paraphrase a text, each paraphrase is more similar to the one made two steps earlier. 
%This implies that the nth paraphrase exhibits higher similarity with the (n-2)th, (n-4)th, (n-6)th, and so forth.
%The convergence of successive paraphrases is that with the number of paraphrase steps increasing, the resulting text is more certain. 
%Meanwhile, the perplexity of paraphrases shows a decreasing trend and eventually converges to a specific value.




%The periodicity of successive paraphrases indicates that when you repeatedly paraphrase a text, the $n$th paraphrase has a higher similarity with the $(n-2)$th, $(n-4)$th, $(n-6)$th, and so on.


%we sometimes find that the paraphrased texts are only slightly refined, while at other times, they differ significantly from their original form.



%Successive paraphrases are iteratively paraphrased texts. 


%Paraphrase application
%Successive Paraphrase

%figure

%Current Research situation -> unique pattern of successive paraphrase,  interesting!

% In this paper

==> article/introduction_v4.tex <==
\section{Introduction}

Paraphrases are different expressions that carry the same meanings \citep{bhagat2013what}.
Paraphrasing tools are frequently used to enhance written material, especially by individuals who are not native speakers~\cite{motlagh_impact_nodate,roe_what_2022,kim_how_2024}.
Moreover, paraphrasing is crucial for data augmentation in situations with limited resources~\cite{okur_data_2022,sobrevilla_cabezudo_investigating_2024}.
The advancement of large language models (LLMs) ~\citep{touvron2023llama2openfoundation,alpaca,gpt3,gpt4} has enabled LLM-based paraphrasing to achieve comparable or even superior results to human performance. 
These models exhibit robust generalization capabilities across text lengths and domains.
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{latex/article/figures/intro_v4.pdf}
    \caption{An illustration of successive paraphrasing using GPT-4o-mini is presented. Here, $T_0$ denotes the original human-written text, while $T_i$ indicates the i-th round of paraphrases. The nodes depicted in the lower section represent valid paraphrases for the input sentence, with distance reflecting textual variation. Successive paraphrases generated by LLMs are confined to alternating between two limited clusters, represented as blue and orange nodes.} 
    \label{figs:intro}
\end{figure}
% A few years ago, models like Parrots \cite{} and Dipper \cite{} primarily focused on sentence-level paraphrasing. However, when dealing with longer contexts, they needed to split the text into individual sentences, paraphrasing each one separately\cite{}. This approach often led to inconsistencies in their output. Moreover, in certain scenarios, their performance fell short of expectations\cite{}.
% Currently, with the advancement of large language models (LLMs) ~\citep{llama,gpt3,gpt4}, paraphrasing has entered a new era, with many paraphrase tools powered by LLMs emerging. The stability of paraphrase quality has greatly improved, and the scope of paraphrasing has expanded from the sentence level to the paragraph level \cite{}.

% Due to the enhanced stability of quality and the inherent nature of paraphrasing, it is intuitive to perform recursive paraphrasing (RP) on texts.
% \citeauthor{can_ai} investigates how RP can evade current AI text detection methods, while \citeauthor{ship} discusses the impact of RP on determining authorship. Compared to these works, we are more interested in the characteristics of RP itself.

Paraphrasing, however, can extend beyond a single transformation. 
A natural next step—successive paraphrasing—asks an LLM to iteratively rephrase its own outputs over multiple rounds~\cite{can_ai,ship}, as shown in Figure~\ref{figs:intro}.
Intuitively, this iterative setup should yield a growing tapestry of linguistic variety. 
With each iteration, the available textual space theoretically expands, promising an exploration of increasingly diverse phrasings.
As the sequence length increases, so does the textual space of potential paraphrases.
Analogous to how widening beam size expands a search space~\cite{Holtzman2020The,huang-etal-2023-affective,meister-etal-2023-locally}, successive paraphrasing can be viewed as a depth-first traversal that enriches textual diversity.




Yet, in practice, these expectations are not fully met. 
In this work, we leverage successive paraphrasing as a lens to examine a phenomenon we term \textbf{generation momentum}—\textit{the tendency of LLMs to self-reinforce and stabilize around particular outputs}. 
Despite the large theoretical space of valid paraphrases, empirical results demonstrate that LLMs repeatedly converge onto a limited set of solutions, as depicted in Figure~\ref{figs:intro}. 
Rather than spiraling outward into new linguistic territory, the iterative paraphrasing loop settles into a pattern of recurring outputs. 
Compared with explicit generation repetition~\cite{see_get_2017,liu_text_2019,fu2020a}, this effect is subtle: it may not manifest as obvious verbatim repetition, but it manifests as paraphrases that structurally and semantically recur in a cyclical pattern. 
Although earlier work has highlighted explicit forms of repetition and degeneracy in LLM outputs~\cite{xu_learning_2022,yan2024understanding}, what we find here is a more implicit and insidious form of repetition. 
By recursively paraphrasing their own paraphrases, LLMs reveal a hidden attractor—an oscillation between a small set of paraphrastic forms—exposing the generation momentum that constrains their creative space.



% In this work, we systematically study the behavior of LLMs in successive paraphrasing.
% Despite the theoretical potential for rich diversity, our empirical observations show that LLMs tend to reinforce their own prior outputs, leading to convergence and limited variation over successive iterations. 
% This observation is consistent with prior research indicating that LLMs have a tendency to produce explicitly repetitive content due to their self-reinforcing nature~\cite{xu_learning_2022,yan2024understanding}.
% %In contrast, we introduce the task of successive paraphrasing as a means to examine the generative momentum of large language models.
% In contrast, the phenomenon introduced here is the implicit repetition problem, which highlights the limited capabilities of LLMs in paraphrasing. 
% Understanding this behavior and mitigating its effects is crucial for tasks that demand high levels of linguistic diversity and creativity.

% data curation & exp


% To accomplish this, we first compile a diverse collection of human-authored texts across various writing tasks~\cite{li-etal-2024-mage}. We then use a set of open-source and commercial LLMs to iteratively paraphrase these texts over 15 successive rounds and quantify the text variation using normalized Levenshtein distance.
% % To quantify the variation between paraphrases, we apply the normalized Levenshtein distance. 
% Our empirical results reveal an increasingly evident cyclic pattern as paraphrasing progresses, with the generated paraphrases becoming more similar to those produced two iterations prior. 
% This 2-period cycle consistently appears across different models, text lengths, and tasks. 
% This unexpected finding challenges the intuition that longer texts (e.g., a 140-word paragraph) should theoretically allow for numerous valid paraphrases, far exceeding the mere two recurring options observed, as shown in Figure~\ref{figs:intro}.


To investigate this phenomenon, we first collect a diverse set of human-authored texts spanning multiple tasks and domains (Li et al., 2024). 
We then task a range of open-source and commercial LLMs with 15 rounds of successive paraphrasing and measure the textual variation using normalized Levenshtein distance. 
Surprisingly, the results show the emergence of a 2-period cycle, wherein each newly generated paraphrase closely resembles the one generated two steps earlier. This pattern persists across different models, text lengths, and tasks. The existence of such a low-order periodicity challenges our intuition: given the rich combinatorial possibilities of longer texts, one would expect a vast array of valid paraphrases rather than an iterative ping-pong between only two recurrent forms as shown in Figure~\ref{figs:intro}.


To further understand this cyclical convergence, we analyze the perplexity of LLMs as paraphrasing unfolds. We observe that with each iteration, the models become more certain about their next outputs, reinforcing prior paraphrases and narrowing the space of possibilities. This self-reinforcing loop—where outputs at one step guide the next step’s generation—creates a kind of gravitational pull. We call this self-sustaining pattern “generation momentum” because it describes how the paraphrasing process, once in motion, builds inertia that resists deviation from previously explored solutions. Under these conditions, the LLM’s “optimal” behavior is to stabilize around a small set of solutions, yielding the observed 2-periodicity.

We then probe the limits of this phenomenon through multiple angles. 
Introducing variability into the iterative process, such as alternating models or prompts, cannot mitigate periodicity. 
Adjusting temperature settings also influences the cycle, but simply increasing randomness does not suffice; overly high temperatures produce nonsensical outputs rather than unlocking sustained diversity. 
Moreover, the observed cyclical pattern extends beyond paraphrasing tasks. 
It appears in any invertible task—one where re-deriving a previous input from a given output is plausible—indicating that the revealed generation momentum is a more general characteristic of LLM behavior. 
% Additional experiments demonstrate that what variation does occur often focuses on swapping synonyms rather than altering deeper structural elements of the text (Section 5.5).
Finally, we propose a straightforward mitigation strategy that breaks this cycle while preserving semantic integrity.
% By addressing the root cause—LLMs’ self-reinforcing tendencies—such methods can restore the intended richness and variety of paraphrasing tasks.
In summary, this work uses successive paraphrasing as a proxy to illuminate the internal dynamics, or generation momentum, that shape LLM outputs. Although LLMs are lauded for their expansive capabilities, we find that when left to iterate on their own outputs, they gravitate towards periodic convergence rather than sustained exploration. Understanding this phenomenon and identifying ways to counteract it is crucial, not only for paraphrasing tasks but also for broader applications where genuine diversity and creativity are desired.










% Inspired by previous research on repetitive text generation~\cite{xu2022learningbreakloopanalyzing}, we investigate the perplexity of the LLMs during successive paraphrasing rounds.
% We observe that as the paraphrasing process continues, LLMs grow more confident when generating new paraphrases based on their previously generated outputs. 
% Concurrently, these models demonstrate heightened confidence in reproducing earlier paraphrases when conditioned on their current outputs.
% This self-reinforcing feedback loop leads to an increasing determinism in the LLMs' generations, thereby significantly constraining variation in paraphrasing.
% Given that paraphrasing inherently demands significant textual diversity, the model's optimal solution under this self-reinforcing behavior is to alternate between the two most likely paraphrases, thus resulting in the observed 2-periodicity.


%To further understand this phenomenon, We investigate the periodicity from many aspects.
%We introduce variability by randomly selecting LLMs or prompts at each step.
%The results show that introducing more variations during paraphrasing can alleviate the periodicity.
%Also, we measure the periodicity of successive paraphrasing in different temperature settings.
%However, raising the temperature alone does not completely prevent the periodicity; instead, it forces the model to produce nonsensical responses when the temperature is too high.
%Besides, This 2-periodicity phenomenon is not limited to paraphrasing, all tasks with an invertible nature, which ensures that the recurrence of the previous response in the next step is reasonable, could perform this in LLMs.
%Moreover, We confirm that rephrasing the paraphrases generated by LLMs always results in synonym substitution rather than altering the structure of the text, through a series of perturbation experiments in section \ref{sec:history}.
%Furthermore, this periodicity can also be changed manually by providing historical paraphrases.
%Finally, we provide an easy way to alleviate this periodicity, while keeping the meaning preserving well.

% To gain a deeper understanding of this phenomenon, we examine the periodicity from multiple perspectives. Specifically, we introduce variability by randomly selecting different LLMs or prompts at each step. The results demonstrate that increasing variability during paraphrasing can mitigate the observed periodicity. Additionally, we assess the periodicity of successive paraphrasing under varying temperature settings. However, merely increasing the temperature does not entirely eliminate periodicity; instead, excessively high temperatures lead the model to generate nonsensical responses. Furthermore, this 2-periodicity is not confined to paraphrasing tasks alone; it extends to any task with an invertible nature, which ensures that the recurrence of previous responses in subsequent steps is justifiable. Moreover, we establish that rephrasing paraphrases generated by LLMs predominantly results in synonym substitution, rather than altering the underlying structure of the text, as demonstrated through a series of perturbation experiments in Section \ref{sec:history}. Finally, we propose a simple approach to alleviate periodicity, while effectively preserving the meaning of the original text.

%Providing historical paraphrases can alter the period in paraphrasing. If we give one previous iteration and rephrase the current paraphrase, the next paraphrase should differ from both previous ones. In this case, the period becomes two, as shown in \ref{sec:history}.


%In Section \ref{sec:beyond paraphrasing}, we present four typical tasks—polishing, style transfer, translation, and clarification—each of which demonstrates the 2-periodicity phenomenon.

% Paraphrasing
%Rephrasing the paraphrases generated by LLMs always results in synonym substitution rather than altering the structure of the text.
%We independently apply three types of perturbations—synonym substitution, word swapping, and random insertion and deletion—throughout the entire generation process.
%The results indicate that synonym substitution has little impact on periodicity, compared to word swapping.
%Providing historical paraphrases can alter the period in paraphrasing. If we give one previous iteration and rephrase the current paraphrase, the next paraphrase should differ from both previous ones. In this case, the period becomes two, as shown in \ref{sec:history}.



%3-periodicity


% Generalization Analysis
%We further discuss this 2-periodicity in terms of text length, tasks, generation settings, perturbation, and finally the methods to mitigate this phenomenon.

%Further experiments demonstrate that the observed 2-periodicity is independent of text length. Even as text length increases, the 2-periodicity remains consistent with that of a single sentence.
%What's more, changing models or prompts have a slight impact on this phenomenon. In fact, our experiments show that these LLMs tend to generate similar paraphrases, as shown in figure\ref{figs:PPL_conditioned_Llama3}.
%Additionally, this phenomenon is prevalent in other invertible tasks, including polishing, translation, style transfer, and clarification, as detailed in Section \ref{sec:beyond paraphrasing}.
%Moreover, when LLMs become trapped in this cycle, increasing randomness has minimal impact on escaping it.
%Forcing it to generate more diverse paraphrases may result in nonsensical responses.
%This indicates a concentrated distribution when LLMs are caught in this state.
%Besides, after investigating three types of perturbations during paraphrasing—synonym replacement, word swapping, and random insertion and deletion, as described in \cite{wei-zou-2019-eda}—the results indicate that LLMs primarily perform synonym replacements for words or phrases, except for the initial paraphrasing.
%Expanding our discussion, we consider the impact of historical paraphrases and argue that providing a paraphrase from a previous step results in 3-periodicity in the current step, as confirmed by our experiments.
%Finally, we propose methods to mitigate this phenomenon based on our findings.
%----------------------------------------------------------



%----------------------------------------------------------









%Based on our analysis, we identify other tasks that exhibit the same periodicity as paraphrasing, including polishing, translation, style transfer, and clarification (see \ref{sec:beyond paraphrasing}). 

%We further explore the 2-periodicity phenomenon from multiple angles. 
%First, we demonstrate that text length has minimal impact on this phenomenon; even as text length increases, the 2-periodicity remains similar to that of a single sentence. 
%Next, we identify other tasks that exhibit the same periodicity as paraphrasing, including polishing, translation, style transfer, and clarification (see \ref{sec:beyond paraphrasing}). 
%In addition to text length and task influences, we find that increased randomness has little effect on this phenomenon, highlighting the sharp distribution of LLMs in the paraphrases. 
%We also investigate three types of perturbations during paraphrasing: synonym replacement, word swapping, and random insertion and deletion, as described in \cite{wei-zou-2019-eda}. The result indicates that LLMs primarily perform synonym replacements for words or phrases, except for the initial paraphrasing.
%Expanding our discussion, we consider the impact of historical paraphrases and discover that providing a paraphrase from a previous step results in 3-periodicity in the current step, as confirmed by our experiments.
%Finally, we propose methods to mitigate this phenomenon based on our findings.


%In summary, we discuss an interesting periodicity with the help of paraphrasing in LLMs.
%Unlike explicit text repetition in neural language generation, this periodicity reflects an implicit repetition, where LLMs regenerate previous paraphrases without it being provided as input.
%Meanwhile, this phenomenon is not limited to paraphrasing.
%It is the external manifestation of the self-reinforcing nature existing in LLMs.
%Compared to previous studies, our finding provides a novel perspective on this nature of LLMs, and reveals the limited capabilities of LLMs in generating diverse responses.


% In summary, we explore an intriguing phenomenon of paraphrasing in LLMs. During successive paraphrasing, LLMs often reproduce earlier paraphrases rather than generating novel variations. This tendency is not confined to paraphrasing alone but is prevalent across other invertible tasks. Our study identifies the root cause of this periodicity as the self-reinforcing nature of LLMs, raising concerns about their limited expressive capabilities.





% To further understand the reason behind this phenomenon, we analyze how conditional perplexity changes. 
% We find that as the number of paraphrasing steps increases, conditional perplexity and the diversity between sampled paraphrases decreases until they converges at a certain value, which we name convergence.
% We also observe a correlation between convergence and periodicity, and we believe that it is convergence leads to periodicity in recursive paraphrasing.
% Besides sufficient experiments, we give both intuitive and mathematical perspectives to support our opinion. Based on our findings, we expand our experiments to other tasks that we believe may exhibit similar characteristics to recursive paraphrasing. 
% The results from these tasks also strongly support our findings.

% findings

% extension


% What will happen if we recursively paraphrase a text multiple times? 
% Given a long text, there are many expressions that convey the same meaning. 
% While keeping the meaning unchanged, can LLMs explore all expressions during recursive paraphrasing, or do they simply remain unchanged as the number of paraphrase steps increases?
% To answer this question, We design a series of experiments and find an interesting phenomenon.
% When we conduct recursive paraphrasing, it appears that the paraphrases keep switching between two states. Specifically, the paraphrase at the current step is much more similar to the paraphrase from two steps prior, which we refer to as periodicity.




% It appears that LLMs have momentum when conducting recursive tasks, which leads them to become trapped in a suboptimal state reflected by convergence.
% To explore the stability of this phenomenon, we designed perturbation experiments that include alternating models and prompts, synonym replacement, as well as random swapping, insertion, and deletion during recursive paraphrasing. The results show that while alternating models and prompts still result in periodic behavior during recursive paraphrasing, random swapping, insertion, and deletion lead to periodicity degradation and loss of similarity. Synonym replacement, on the other hand, causes only slight periodicity degradation.
% Finally, we propose a method to mitigate generation momentum by sampling multiple paraphrases and selecting the one with the highest conditional perplexity.

% Humans continuously change, with each individual expressing themselves uniquely, shaped by their diverse life experiences. In comparison, LLMs exhibit limitations in maintaining diverse expressions while conveying the same meaning. Although there are various types of LLMs, they tend to produce similar expressions when performing recursive tasks.
% Consequently, we can more accurately determine whether the text was generated by LLMs if we provide the related question.
% We believe this represents a homogeneous problem, both in terms of generation and across different LLMs.
% However, does enhancing expressive diversity conflict with LLMs' ability to answer questions correctly?
% We consider this a valuable question that needs to be explored in the future.




















%Alternating Models and Prompts
%Human Intervention
%Mitigating Generation Momentum











%However, some research also poses that potential misuse of paraphrasing might lead to plagiarism and the spread of fake news. 
%Besides, these texts paraphrased by LLMs might suffer from hallucinations\cite{} and factual errors\cite{}.
%Although there has been a considerable amount of work focusing on paraphrasing, most of it only considers text that has been paraphrased once.
%In the real world, due to the widespread use of LLMs, any text you read on the internet might have been edited and paraphrased multiple times by various individuals for different reasons,    a process we refer to as successive paraphrasing.
%Based on our intuition and daily use of LLMs, we have noticed that successive paraphrasing exhibits some unique properties which raise our great interest.


==> article/tables/main_periodicity.tex <==
\begin{figure}
    \centering
    \begin{s}
    \includegraphics[width=0.5\linewidth]{}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}
